SN2019dge: a Helium-rich Ultra-Stripped Envelope Supernova

We present observations of ZTF18abfcmjw (SN2019dge), a helium-rich supernova with a fast-evolving light curve indicating an extremely low ejecta mass ($\approx 0.3\,M_\odot$) and low kinetic energy ($\approx 1.2\times 10^{50}\,{\rm erg}$). Early-time (<4 d after explosion) photometry reveal evidence of shock cooling from an extended helium-rich envelope of $\sim0.1\,M_\odot$ located at $\sim 3\times 10^{12}\,{\rm cm}$ from the progenitor. Early-time He II line emission and subsequent spectra show signatures of interaction with helium-rich circumstellar material, which extends from $\gtrsim 5\times 10^{13}\,{\rm cm}$ to $\gtrsim 2\times 10^{16}\,{\rm cm}$. We interpret SN2019dge as a helium-rich supernova from an ultra-stripped progenitor, which originates from a close binary system consisting of a mass-losing helium star and a low-mass main sequence star or a compact object (i.e., a white dwarf, a neutron star, or a black hole). We infer that the local volumetric birth rate of 19dge-like ultra-stripped SNe is in the range of 1400--8200$\,{\rm Gpc^{-3}\, yr^{-1}}$ (i.e., 2--12% of core-collapse supernova rate). This can be compared to the observed coalescence rate of compact neutron star binaries that are not formed by dynamical capture.

==> tables/tab_compare.tex <==
\begin{deluxetable*}{lllll}[htbp!]
	\tablecaption{Summary of Subluminous Fast Transient. \label{tab:compare}}
	\tablehead{
		\colhead{Name}   
		& \colhead{Redshift} 
		& \colhead{Host} 
		& \colhead{Offset (kpc)}   
		& \colhead{Reference}   
	}
	\startdata
	SN\,2002bj & 0.012   & NGC 1821 (small barred irregular galaxy, $D\sim$1.1'') & 1.8\,kpc \\
	SN\,2005ek & 0.016 & UGC 2526 (edge-on spiral galaxy of morphology Sb) & 30\,kpc \\
	SN\,2010X &  0.015  & NGC 1573A (small spiral galaxy, $D\sim$1.6'') & 2.3\,kpc\\
	%PTF\,10iuv & 0.025?   &  Galaxy cluster with early-type and late-type galaxies   & $\geq 37$\,kpc  \\
	iPTF\,14gqr & 0.063 & IV Zw 155 (a tidally interacting spiral galaxy) & 29\,kpc & \citet{De2018} \\
	SN\,2019bkc & $\sim$0.02   & maybe NGC 3090 (giant elliptical in the MKW1 galaxy group) 
	&$\sim94.6$ & \citet{Chen2019}  \\
	SN2019dge & 0.021 & SDSS J17$+$50 (small) & 0.06 kpc & This work \\
	\enddata
	%\tablecomments{Reference: SN\,2019bkc \citep{Prentice2019}, iPTF\,14qgr \citep{De2018}, 
	%OGLE13-079 \citep{Inserra2015}, SN\,2002bj 
	%\citep{Poznanski2010}, SN\,2010X \citep{Kasliwal2010}, SN\,2016hnk \citep{Galbany2019}, 
	%AT\,2018dge (Yao in prep), SN\,2005ek \citep{Drout2013}.}
\end{deluxetable*}

